A User Model for Information Erasure

Hunt and Sands (ESOP'08) studied a notion of information erasure for systems which receive secrets intended for limited-time use. Erasure demands that once a secret has fulfilled its purpose the subsequent behaviour of the system should reveal no information about the erased data. In this paper we address a shortcoming in that work: for erasure to be possible the user who provides data must also play his part, but previously that role was only specified informally. Here we provide a formal model of the user and a collection of requirements called erasure friendliness. We prove that an erasure-friendly user can be composed with an erasing system (in the sense of Hunt and Sands) to obtain a combined system which is jointly erasing in an appropriate sense. In doing so we identify stronger requirements on the user than those informally described in the previous work.

==> eptcsdata.tex <==
\providecommand{\event}{M. Boreale, S. Kremer (Eds.):\\
 Security Issues in Concurrency (SecCo'09)}
\providecommand{\volume}{7}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{16}
\providecommand{\eid}{2}
\pdfoutput=1

